PaC-trees: Supporting Parallel and Compressed Purely-Functional Collections

Many modern programming languages are shifting toward a functional style for collection interfaces such as sets, maps, and sequences. Functional interfaces offer many advantages, including being safe for parallelism and providing simple and lightweight snapshots. However, existing high-performance functional interfaces such as PAM, which are based on balanced purely-functional trees, incur large space overheads for large-scale data analysis due to storing every element in a separate node in a tree. This paper presents PaC-trees, a purely-functional data structure supporting functional interfaces for sets, maps, and sequences that provides a significant reduction in space over existing approaches. A PaC-tree is a balanced binary search tree which blocks the leaves and compresses the blocks using arrays. We provide novel techniques for compressing and uncompressing the blocks which yield practical parallel functional algorithms for a broad set of operations on PaC-trees such as union, intersection, filter, reduction, and range queries which are both theoretically and practically efficient. Using PaC-trees we designed CPAM, a C++ library that implements the full functionality of PAM, while offering significant extra functionality for compression. CPAM consistently matches or outperforms PAM on a set of microbenchmarks on sets, maps, and sequences while using about a quarter of the space. On applications including inverted indices, 2D range queries, and 1D interval queries, CPAM is competitive with or faster than PAM, while using 2.1--7.8x less space. For static and streaming graph processing, CPAM offers 1.6x faster batch updates while using 1.3--2.6x less space than the state-of-the-art graph processing system Aspen.

==> algo-old.tex <==

\hide{  % now in betterworkbound.tex
\subsection{Set Algorithms with Better Work Bound}
\label{app:setalgo}
In this section, we describe the set algorithms with better work bound. The algorithm is shown in \cref{fig:setcode} as \texttt{union\_}.

The general idea is to avoid folding and unfolding \simple{} trees
during the \union{} algorithm. In particular, we hope each
\blockednode{} is folded and unfolded $O(1)$ times during the entire
\union{} algorithm. To ensure this, we implemented a special base case for
the set algorithms. We show the code for \union{} in
\cref{fig:setcode}, the other two are similar. The base case will
explicitly determine if the current input is a \blockednode{}. If any
of them is, it will be \exploded{} directly. In the subsequent
\join{}, we will pass an extra parameter to indicate that the tree is
already \exploded{}, and thus there is no need to fold or unfold them
again in this \join{} algorithm. This parameter is the last parameter
of the \join{} algorithm in \cref{fig:codeappjoin}. It is set to
\false{} by default, which makes it exactly the same as the version in
\cref{fig:mainalgo}. When it is set to \true{}, the \join{} algorithm
will never \fold{} any node. Instead, at the end of the base case, the
entire result tree will be fixed using \refold{} (Line
\ref{union:refold}), which traverses the tree and folds any subtree of
size $B$ to $2B$ back to blocks.



\subsection{Proofs for the More Efficient Set Algorithms}
\label{app:setproof}

In this section, we will prove \cref{thm:unionwork}.
\setefficient*

As the span bound is not affected, we will only show the new proof for
the work here. First, note that total work for each of these
algorithms can be considered as several parts:

\begin{enumerate}[label=(\arabic*).]
  \item \label{item:unfold} all work done by \unfold{} operations in the base cases, including possibly those in \tsplit{} and \join{} (or \joinTwo{}) function calls, denoted as \emp{unfold work},
  \item all work done by \refold{} operations, denoted as \emp{refold work},
  \item all work done by \tsplit{} operations except for the \unfold{} work in base cases (already charged in \ref{item:unfold}, denoted as \emp{split work},
  \item all work done by \join{} or \joinTwo{} operations, denoted as \emp{join work}.
\end{enumerate}

We note that all the rest of the cost can be asymptotically bounded by the above four categories of work.

One observation is that the split work and unfold work are identical
among the three set algorithms. This is because the three algorithms
behave the same on the way down the recursion when doing \tsplit{}s,
and algorithms only differ in what they do at the base case and on the
way up the recursion when they join back.

We start with some notation.  We follow some the notation used in \cite{blelloch2016just}.
Throughout the section, we use \op{} to denote the algorithm or function call on \union{}, \intersection{} or \difference{}, and use \opbase{} to denote the corresponding base case algorithm or function call (using the unfolded version).
In these three algorithms, the first tree ($T_1$) is split by the keys in the second tree ($T_2$).  We
call $T_1$ the \emp{decomposed tree} and $T_2$ the
\emp{pivot tree}, denoted as $T_d$ and $T_p$ respectively.  The returned
tree of the algorithms is denoted as $T_r$.
We use $m=\min(|T_p|, |T_d|)$ and
$n=\max(|T_p|,|T_d|)$.
We denote the subtree rooted at $v \in T_p$ as $T_p(v)$, and the tree
of keys from $T_d$ that $v$ is operated with as $T_d(v)$ (i.e.,
\op$(v,T_d(v))$ or \opbase$(v,T_d(v))$ is called at some point in the algorithm.
This essentially means that $v$'s subtree in $T_p$ is processed with the tree $T_d(v)$ in a recursive call.
Note that $T_d(v)$ may not be a subtree in $T_d$, but is a tree of keys as a subset of $T_d$. We call such $T_d(v)$ a \emp{\subsettree{}} of the \decomposedtree{} $T_d$. We say $v\in T_p$ \emp{\dealswith} $T_d(v)$.
For $v \in T_p$, we refer to $|T_d(v)|$ as its \emp{splitting size}.

\begin{lemma}
The refold work can be asymptotically bounded by the unfold work.
\end{lemma}
\begin{proof}
  We note that during the process of tracking down the tree, we will
  refold the subtree if and only at least a subset of it was
  previously unfolded at some point in this algorithm. Since \refold{}
  costs $O(\B)$ work, it can be asymptotically bounded by the
  corresponding \unfold{} function invoked previously.
\end{proof}

\begin{theorem}
\label{thm:appjoinlarger}
For each function call to \op{} on
trees $T_p(v)$ and $T_d(v)$, the work done the \join{} (or \joinTwo{})
is asymptotically bounded by the work done by \tsplit{}.
\end{theorem}
\begin{proof}
In the following, we use $P$ and $D$ to denote
$T_p(v)$ and $T_d(v)$, respectively, for simplicity. Assume the return value is $R$. First of all, the work of \tsplit{} is $\Theta(\log |D|+\B)$.

For \intersection{} or \difference{}, the work of \join{} (or \joinTwo{})
is $O(\log|R|+\B)$.
Notice that \difference{} returns the keys in $D\backslash P$. %\yihan{need to verify this.}
Thus for both \intersection{} and \difference{} we have $R\subseteq D$. Therefore $|R|\le |D|$, which means the work done by \join{} or \joinTwo{} is no more than the work done by \tsplit{}.

For \union{}, first of all, we always call \join{} instead of \joinTwo{}. If $|P|\le |D|$, then $|R|\le 2|D|$.
\join{} costs work $O(\log |R|+B)=O(\log |P|+B)$, which is no more than $\Theta(\log |D|+\B)$.

Consider $|P|>|D|$. The subtrees $\lc(P)$ and $\rc(P)$,
which are used in the recursive calls, have size at least $\alpha|P|$ and at most $(1-\alpha)|P|$.
After combining with a subset of elements in $D$ (which has size smaller than $|P|$), the return value of each recursive call should have size at least $\alpha|P|$ and $(2-\alpha)|P|$. Denote these two trees from recursive calls as $t_l$ and $t_r$, respectively.
Note that $\alpha$ is a constant, so the difference of size between $t_l$ and $t_r$ is also a constant.
WLOG assume $|t_l|\ge |t_r|$. In the following, we discuss different cases of whether $t_l$ and $t_r$ are \composite{} or \simple{} trees.
We will show that, in all cases, joining $|t_l|$ and $|t_r|$ has work $O(\log |D|+\B)$.

\begin{enumerate}
  \item When both $t_l$ and $t_r$ are \simple{} trees. From \cref{lem:joincost}, \join{} costs $O(\B)$ work.
  \item When both $t_l$ and $t_r$ are \composite{} trees. From \cref{lem:joincost}, \join{} costs $O(\log \frac{|r_l|}{|t_r|})=O(1)$ work.
  \item When $t_l$ is a \composite{} tree, but $t_r$ is a \simple{} tree. This means that $|t_l|>\B$ and $|t_r|\le \B$.
  From \cref{lem:joincost}, \join{} costs $O\left(\B + \log\frac{|t_l|}{\B}\right)$ work. Note that, as stated above, $|t_r|\ge \alpha|P|$. Considering $|t_r|\le B$, we know that $|P|=O(B)$, which also indicates $|t_l|=O(\B)$. Plug this into the work of \join{} $O\left(\B + \log\frac{|t_l|}{\B}\right)$, we can get the bound $O(\B)$.
\end{enumerate}

In summary, in all cases, the work of \join{} or \joinTwo{} is asymptotically bounded by the corresponding \tsplit{} function.
\end{proof}

From the above two lemmas, we have that the total work of \op{} is
asymptotically bounded by the split work and unfold work. Next, we
prove the bounds for split work and unfold work, respectively.


\begin{lemma}
The unfold work is $O(\min(m\B, n))$.
\end{lemma}
\begin{proof}
  First, note that in our unfolded version of base cases, any \block{}
  needs to be unfold at most once. Each time the algorithm hits a
  \blockednode{s}, it unfold the entire subtree in $O(B)$ time.

  If $|T_p|=m$, we note that there are at most $m/\B$ \blockednode{s}
  in $T_p$ that needs to be unfolded, so the total work to unfold
  $T_p$ is $O(m)$. Each of the $O(m)$ entries in $T_p$ will cause an
  \unfold{} on at most one \block{} in $T_d$. Therefore, the total
  work to unfold $T_d$ is $O(m\B)$. On the other hand, note that each
  \block{} in $T_d$ can be unfolded at most once, which also means
  that the work of unfolding $T_d$ is $O(n)$. In summary, the work of
  all \unfold{} functions is $O(\min(m\B, n))$.

  If $|T_d|=m$ and $|T_p|=n$, there will be at most $O(m)$ nodes in
  $T_p$ used to \dealwith{} a \subsettree{} in $T_d$. Since $|T_d|=m$,
  the total work of unfolding $T_d$ is at most $O(m)$. Based on the
  same argument as above, the total work of unfolding $T_p$ is
  $O(m\B)$ because at most $O(m)$ \unfold{} functions are invoked, and
  is also $O(n)$ because there are at most $O(n)$ entries in $T_p$.
  The total work is also $O(\min(m\B, n))$.
\end{proof}



\begin{lemma}[Split work on \exploded{} trees]
\label{lem:appPAMsplit}
The total split work done on two \exploded{} weight-balanced trees of sizes $n$ and $m\le n$ is $O\left(m\log \frac{n}{m}\right)$.
\end{lemma}
This directly follows \cite{blelloch2016just}.

\begin{lemma}
The total \tsplit{} work is $O\left(m\log \frac{n}{m}+\min(m\B,n)\right)$.
\end{lemma}
\begin{proof}
  The total work for \tsplit{} functions can be viewed as two parts:
  the total work to done by \tsplit{} functions to traverse and split
  non-\blockednode{s}, and the work to expose and split the
  \blockednode{s}. Note that here ``non-\blockednode{s}''
  include both \internalnode{s} in \composite{} trees, and all the
  nodes in \exploded{} trees.

  We first note that in the base cases, the
  \tsplit{}$(\cdot,\cdot,\true)$ function must be working on a
  \exploded{} tree. As a result, the total work to traverse and split all non-\blockednode{s} can be asymptotically bounded by the split work considering if both $T_p$ and $T_d$ are fully expanded. This cost can be computed by \cref{lem:appPAMsplit}, which is $O\left(m\log \frac{n}{m}\right)$.

  We then consider all work done by the \tsplit{} functions on \blockednode{s} in the non-base cases. We will show it is $O(\min(mB,n))$.
  Note that in each \tsplit{}, this happens at most once, costing $O(B)$ work.
  If $|T_p|=m$, there can be $O(m/\B)$ such \tsplit{} function calls in the non-base cases, and thus the total non-base case split work on \blockednode{s} is $O(m)$.

  If $|T_p|=n$, we discuss in two cases. If $n/\B\le m$, there are $O(n/\B)$ \internalnode{s} in $T_p$, and thus there can be at most $O(n/\B)$ \tsplit{} calls. Therefore the total work in this case is $O(n)$, which is also $O(\min(mB,n))$. If $n/\B > m$, there are at most $O(m)$ such \tsplit{} function calls, since there are only $m$ nodes in $T_d$. In this case, the total work of this part is $O(m\B)$, which is also $O(\min(mB,n))$.
\end{proof}
%  We first prove that the total work to split all \simple{} trees is $O(m\B)$. We can discuss in two cases:
%  \begin{enumerate}
%    \item If $|T_p|=m$ and $|T_d|=n$, it means that there can be at most $m$ splits. Each \tsplit{} function splits at most one \compressednode{}. So the total cost is at most $O(m\B)$.
%    \item If $|T_p|=m$ and $|T_d|=n$, then at most $O(m)$ nodes in $T_p$ will be used to split a \subsettree{} in $T_p$. From the same argument as above, the total cost is $O(m\B)$.
%  \end{enumerate}
%
%  We then prove that the total work to split all \composite{} trees is $O\left(m\log \frac{n}{m\B}\right)$. From \cref{thm:splitcost}, we know that cost is $O(\log\frac{|T|}{\B}+\B)$. Therefore, we can also split the cost into two parts: the cost to split the \compressednode{s}, which is $O(\B)$ per \tsplit{} function, and those to search and reconnect the \internalnode{s} in $T$.

}


\hide{
\subsection{some lemmas}
\yihan{some lemmas that may not be useful for the final proof.}
\begin{lemma}
The expose work is $O(m)$.
\end{lemma}
\begin{proof}
  Note that all \expose{} functions in \op{} happens after checking if $T_2$ is not a \blockednode{}. Also, in the corresponding base case functions, \expose{} is called on $T_2$ only after $T_2$ is unfolded. Therefore, in both cases, the work for such an \expose{} function is a constant. Considering that there can be at most $O(m)$ recursive calls, the total expose work is $O(m)$.
\end{proof}

\begin{lemma}
In a \ourtree{} $T$, all \internalnode{s} form a weight-balanced tree with balance factor $\frac{\alpha}{2-\alpha}$.
\end{lemma}
\begin{proof}
  Consider an \internalnode{} $v$ in a \ourtree{} and its sibling $u$. Denote their parent as $p$. Assume the number of \internalnode{s} in a subtree of $T$ rooted at a node $x$ is $s(x)$. Recall that we use $w(u)$ and $w(v)$ to denote the weight of $u$ and $v$ in the \ourtree{}, respectively.
  Then we have:
  \begin{align*}
    \B(s(u)+1)\le&w(u)\le 2\B(s(u)+1)\\
    \B(s(v)+1)\le&w(v)\le 2\B(s(v)+1)
  \end{align*}
  Denote $\beta = \frac{1-\alpha}{\alpha}$. Considering the weight-balance invariant, we also have $\frac{1}{\beta} w(u)\le w(v)\le \beta w(u)$. If we look at the binary tree $T'$ formed by all the \internalnode{s} in this \ourtree{}, we denote the weight of a subtree in $T'$ rooted at a node $x$ as $w'(x)=s(x)+1$.
  By using the inequations we can get:
  \begin{align*}
  &\B(s(u)+1)\le w(u)\le \beta w(v)\le 2\B\beta(s(v)+1)\\
  %\Rightarrow & s(u)+1 \le \frac{2}{\alpha}(s(v)+1)
  \Rightarrow & w'(u) \ge 2\beta w'(v)\\
  \Rightarrow & w'(v) \le \frac{1}{2\beta+1}w'(p)\\
  \Rightarrow & w'(v) \le \frac{\alpha}{2-\alpha}w'(p)
  \end{align*}
  Since $v$ is either child of $u$, we can also get the symmetric conclusion $w'(v) \ge \frac{2-\alpha}{\alpha}w'(p)$. This shows that $T'$ is a weight-balanced tree with balancing factor $\alpha'=\frac{2-\alpha}{\alpha}$.
\end{proof}

\begin{lemma}
In a weight-balanced tree $T$, we can partition all tree nodes into $l$ layers, such that:
\begin{itemize}
  \item $l=O(\log |T|)$.
  \item For any two nodes $u$ and $v$ in the same layer, $u$ is not the parent of $v$.
  \item The number of nodes in layer $i$, denoted as $s_i$, is no more than $|T|/c^i$ for some constant $c$.
\end{itemize}
\end{lemma}
}



==> coverpage.tex <==
%\begin{center}
%  \Large\textbf{Cover Page}
%\end{center}

Dear Xipeng and Isil,\\

Please find attached the revised version of our PLDI paper (Paper
801). We have made the following changes and modifications which were
not included in the original paper, as per our discussion with the
reviewers:

\begin{itemize}
  \item (Done) Add some comments to discussion/conclusion about ``large internal nodes/higher branching factor to reduce latency'' (review D).
  \item (Done) Add a summary of experiments at the start of that section.
  \item (Done) Fix references for chunked sequences.
  \item (Done) More description of granularity control (review E).
  \item Space permitting, add some ``hello world'' program text illustrating how to use the library. Could also add this in the appendix.

  \item (Done) Clarify the parameters being used in each experiment (review B).
  \item (Done) Clarify: “Regarding the question about L 281 (which theoretical bounds are stronger), we are referencing the bounds for Union/Difference/Intersection for the PAC-tree and C-tree data structures, and will clarify this in the final version.
  \item (Done) Fix units in Figure 15.
\end{itemize}





==> microbench_table.tex <==

\begin{table*}[!t]
\footnotesize
\centering
\begin{tabular}[!t]{lccrrrrrrrrr}
\toprule
\multirow{2}{*}{} & \multirow{2}{*}{$n$} & \multirow{2}{*}{$m$} & \multicolumn{3}{c}{\bf \ourtree{}} &  \multicolumn{3}{c}{\bf \ourtree{} (Diff)} & \multicolumn{3}{c}{\bf \ptree{} (PAM)} \\

& & & $T_{1}$ & $T_{144}$ & {Spd.} & $T_{1}$ & $T_{144}$ & {Spd.} & $T_{1}$ & $T_{144}$ & {Spd.} \\
\midrule
\multicolumn{12}{l}{\textbf{No augmentation}} \\
\midrule
%1618874344      926214369
%1629360096      936700121
{\emph{Size (GB)}}   & $10^{8}$ & ---        & 1.61  & ---     & ---    & 0.926& ---    & ---         & 4.00  & ---    & --- \\
{\emph{Build}}   & $10^{8}$ & ---            & 5.55  & 0.186 & 29.8     & 5.71 & 0.180 & 31.7         & 5.94  & 0.221  & 26.8 \\
{\emph{Union}}   & $10^{8}$ & $10^{8}$       & 5.33  & 0.088 & 60.5     & 6.29 & 0.089  & 70.6        & 8.97  & 0.168  & 53.3 \\
{\emph{Union}}   & $10^{8}$ & $10^{5}$       & 1.09  & 0.021 & 51.9     & 1.28 & 0.022 & 58.1         & 0.206  & 0.0038 & 54.2 \\
{\emph{Intersect}}   & $10^{8}$ & $10^{8}$   & 4.35  & 0.065 & 66.9     & 5.68 & 0.081 & 70.1         & 9.50  & 0.139  & 68.3  \\
{\emph{Difference}}   & $10^{8}$ & $10^{8}$  & 3.00  & 0.055 & 54.4     & 3.55 & 0.056 & 63.3         & 8.17  & 0.123  & 66.4 \\
{\emph{Filter}}   & $10^{8}$ & $10^{8}$      & 0.997 & 0.028 & 3.56     & 1.24 & 0.018 & 68.8         & 1.90  & 0.0524 & 36.2 \\
{\emph{Find}}    & $10^{8}$ & $10^{8}$       & 103   & 1.17 & 88.0      & 125 & 1.23 & 101.6          & 105.5 & 1.05   & 100.4 \\
{\emph{Insert}}  & $10^{8}$ & $10^{6}$       & 0.829 & --- & ---        & 1.42 & ---  & ---           & 0.773 & --- & --- \\
{\emph{Multi-Insert}}  & $10^{8}$ & $10^{8}$ & 18.8  & 0.332 & 56.6     & 19.9 & 0.323 & 0.616        & 9.67  & 0.338  & 28.6  \\
{\emph{Range}}   & $10^{8}$ & $10^{6}$       & 11.5  & 0.318 & 36.1     & 13.1 & 0.226 & 57.9         & 3.77  & 0.0738 & 45.6 \\  % TODO: check by hand
\midrule
\multicolumn{12}{l}{\textbf{With augmentation}}\\
\midrule
{\emph{Size (GB)}} & $10^{8}$ & ---            & 1.63 & ---        & ---    & 0.936 & ---  & ---        & 4.80 & --- & --- \\
{\emph{Build}}   & $10^{8}$ & ---              & 5.66 & 0.197 & 28.7   & 5.84 & 0.186 & 31.3       & 6.48  & 0.246 & 26.3 \\
{\emph{Union}}   & $10^{8}$ & $10^{8}$         & 5.52 & 0.098 & 56.3   & 6.52 & 0.090 & 72.4       & 10.13 & 0.196 & 51.6 \\
{\emph{AugRange}}   & $10^{8}$ & $10^{7}$      & 12.3 & 0.331 & 37.1   & 13.9 & 0.234 & 59.4       & 4.80  & 0.082 & 58.5 \\
{\emph{AugFilter}}   & $10^{8}$ & $10^{8}$     & 12.2 & 0.333 & 36.6   & 13.6 & 0.234 & 58.1       & 4.95  & 0.081 & 61.1 \\
\end{tabular}
\captionof{table}{Microbenchmark results. We fix $B=128$ for both types of \ourtree{s}.}
\label{table:microbench}
\end{table*}

% (10^8, 10^5) only 0.006378 for B=16 (1.67x slower), only 0.008547 for B=32 (2.24x slower).
% 0.004288 for B=4


%\begin{table*}[!t]
%\footnotesize
%\centering
%\begin{tabular}[!t]{lccrrrrrrrrr}
%\toprule
%\multirow{2}{*}{} & \multirow{2}{*}{$n$} & \multirow{2}{*}{$m$} & \multicolumn{3}{c}{\bf \ourtree{}} &  \multicolumn{3}{c}{\bf \ourtree{} (Diff)} & \multicolumn{3}{c}{\bf PAM} \\
%
%& & & $T_{1}$ & $T_{144}$ & {Spd.} & $T_{1}$ & $T_{144}$ & {Spd.} & $T_{1}$ & $T_{144}$ & {Spd.} \\
%\midrule
%\multicolumn{12}{l}{\textbf{No augmentation}} \\
%\midrule
%%1618874344      926214369
%%1629360096      936700121
%{\emph{Size (GB)}}   & $10^{8}$ & ---        & 1.61  & ---     & ---   & 0.926& ---    & ---    & 4.00  & ---    & --- \\
%{\emph{Build}}   & $10^{8}$ & ---            & 6.50  & 0.148  & 43.9   & 7.09 & 0.165  & 42.9   & 5.94  & 0.221  & 26.8 \\
%{\emph{Union}}   & $10^{8}$ & $10^{8}$       & 3.64  & 0.0591 & 61.5   & 5.03 & 0.0713 & 70.5   & 8.97  & 0.168  & 53.3 \\
%{\emph{Intersect}}   & $10^{8}$ & $10^{8}$   & 3.35  & 0.0632 & 53.1   & 4.91 & 0.0903 & 54.3   & 9.50  & 0.139  & 68.3  \\
%{\emph{Difference}}   & $10^{8}$ & $10^{8}$  & 2.39  & 0.0552 & 43.2   & 3.00 & 0.0531 & 56.4   & 8.17  & 0.123  & 66.4 \\
%{\emph{Filter}}   & $10^{8}$ & $10^{8}$      & 0.846 & 0.0153 & 30.0   & 1.04 & 0.0150 & 69.3   & 1.90  & 0.0524 & 36.2 \\
%{\emph{Find}}    & $10^{8}$ & $10^{8}$       & 91.6  & 0.891  & 102.8  & 110  & 1.207  & 91.6   & 105.5 & 1.05   & 100.4 \\
%{\emph{Insert}}  & $10^{8}$ & $10^{6}$       & 0.586 & ---    & ---    & 1.20 & ---  & ---  & 0.773 & --- & --- \\
%{\emph{Multi-Insert}}  & $10^{8}$ & $10^{8}$ & 14.2  & 0.232  & 61.2   & 16.2 & 0.248  & 65.3   & 9.67  & 0.338  & 28.6  \\
%{\emph{Range}}   & $10^{8}$ & $10^{6}$       & 9.18  & 0.200  & 45.9   & 10.8 & 0.163  & 66.2   & 3.77  & 0.0738 & 45.6 \\  % TODO: check by hand
%\midrule
%\multicolumn{12}{l}{\textbf{With augmentation}}\\
%\midrule
%{\emph{Size (GB)}} & $10^{8}$ & ---            & 1.63 & ---    & ---    & 0.936 & --- & ---        & 4.80 & --- & --- \\
%{\emph{Build}}   & $10^{8}$ & ---              & 6.86 & 0.151  & 45.4   & 7.33 & 0.152  & 48.2     & 6.48  & 0.246 & 26.3 \\
%{\emph{Union}}   & $10^{8}$ & $10^{8}$         & 4.21 & 0.0629 & 66.9   & 5.44 & 0.0769 & 70.7     & 10.13 & 0.196 & 51.6 \\
%{\emph{AugRange}}   & $10^{8}$ & $10^{7}$      & 9.34 & 0.219  & 42.6   & 11.3 & 0.184  & 61.4     & 4.80  & 0.082 & 58.5 \\
%{\emph{AugFilter}}   & $10^{8}$ & $10^{8}$     & 9.39 & 0.216  & 43.4   & 11.3 & 0.183  & 61.7     & 4.95  & 0.081 & 61.1 \\
%\end{tabular}
%\captionof{table}{Microbenchmark results.}
%\label{table:microbench}
%\end{table*}


==> old_abstract.tex <==
\begin{abstract}
Ordered (key-value) maps are an important and widely-used data type
in large-scale applications today. There are two major challenges
in these applications. First, they require analyzing data while
undergoing rapid concurrent updates, which creates difficulty both for
efficiency (e.g., non-blocking) and correctness (e.g., atomicity).
They also require high memory usage due to the memory-inefficient data
structures that are commonly used for maps in practice.
%This could highly affect
%performance, and can even make it impossible to get an in-memory
%solution for very large data.

We propose \ourtree{s}, a general-purpose space-efficient
implementation of ordered maps, which support snapshot isolation
(i.e., concurrent operations work on snapshots without interfering
with each other) and efficient parallel batch updates and queries.
\ourtree{s} are inspired by prior work on parallel functional trees,
specifically P-trees (Sun et al.) and C-trees (Dhulipala et al.).
A \ourtree{} is a binary search tree with blocked leaves (possibly
encoded) for space-efficiency.
It is purely functional, which efficiently supports snapshot isolation
to enable atomicity for operations.  \ourtree{s} support parallel bulk
operations such as union, intersection, filter, reduction, and range
queries. These algorithms are both theoretically and practically
efficient and are elegantly integrated in an existing library called
PAM. The algorithms are useful in many applications, e.g., in graph
processing, 2D range queries, 1D interval queries, and inverted
indexes, which we apply \ourtree{s} to and study their performance.


%We have implemented the algorithms and present several experimental
%results.
We implement \ourtree{s} in a parallel library called \cpam{} and
experimentally evaluate our implementation.
This includes a direct comparison to PAM, as well as a study on the
aforementioned applications.
Our experiments show that \ourtree{} operations are generally
competitive with, or faster than PAM due to improved space-efficiency,
and use 2.1--7.8x less space. For graph applications, we achieve
competitive performance to Aspen, and improve the space by 1.1--2.7x.
\end{abstract}



==> proof-old.tex <==
\section{Proofs of Join and Split Algorithms}\label{app:joinsplitproof}

%\subsection{}
In this section, we prove \cref{lem:joincost,thm:splitcost} that we leave out in the main body.

%\begin{theorem}
%\label{lem:joincost}
%Consider a \join{} algorithm on two \ourtree{s} $\Tl$, $\Tr$ and an entry $e$, where $\Tl<k(e)<\Tr$. Let $n=\max(|\Tl|,|\Tr|)$ and $m=\min(|\Tl|,|\Tr|)$.
%If both $\Tl$ and $\Tr$ are \composite{} trees, the algorithm takes $O\left(\log\frac{n}{m}\right)$ work.
%If both $\Tl$ and $\Tr$ are \simple{} trees, the algorithm takes $O(\B)$ time.
%Otherwise, the algorithm takes $O\left(\B + \log\frac{n}{\B}\right)$ time.
%\end{theorem}

\joincost*

\begin{proof}
WLOG, assume $n=|\Tl|\ge|\Tr|=m$. %The other case is symmetric.

For two \composite{} trees, we first prove that \join{} never decompresses a leaf.
%
Note that the algorithm will follow the right spine of the tree until finding a subtree $t$ in $\Tl$ that is balanced with $\Tr$, we will prove that there exist a \internalnode{} $t$ that is balanced with $\Tr$.
This is because as a \composite{} tree, $\Tr$ has size at least $2\B$. Along the right spine of $\Tl$, the smallest \composite{} subtree has size at most $4\B$. For any $\alpha\le 1/3$, we must be able to find a \composite{} subtree in $\Tl$ that is balanced with $\Tr$. This proves that the total number of tree nodes we need to visit on the right spine is $O\left(\log\frac{n}{m}\right)$.

For two \simple{} trees, the work is no more than copying both $\Tl$ and $\Tr$ and concatenating them, which is $O(\B)$ work and $O(\log B)$ span.


If $\Tl$ is a \composite{} tree and $\Tr$ is a \simple{} tree, we need to first follow the right spine to find a \leafnode{} $l$ in $\Tl$, which takes $O\left(\log\frac{n}{B}\right)$ time. Then it combines the \leafnode{} with $\Tr$, which flattens both $l$ ant $\Tr$, concatenates them, and rebalance the result. This process takes no more than $O(B)$ work and $O(\log B)$ span.
\end{proof}

\splitcost*

\begin{proof}
  For a \simple{} tree the cost directly follows the result on \ptree{s}~\cite{blelloch2016just}. For a \composite{} tree, the only difference of \tsplit{} on \ourtree{s} from \tsplit{} on PAM trees is the \unfold{} performed in \expose{} and  \fold{} in \join{}. It takes $O(\log |T|/B)$ steps to reach a \leafnode{}. The \unfold{} function in \expose{} (Line \ref{line:splitexpose}) is performed at most once. For all \join{} calls, at most one on each side can involve a \simple{} tree. So the total overhead is at most $O(\B)$ in work and $O(\log B)$ in span.
\end{proof}



